On The Scalability of P2P Swarming Systems

One of the fundamental problems in the realm of peer-to-peer systems is that of determining their service capacities. In this paper, we focus on P2P scalability issues and propose models to compute the achievable throughput under distinct policies for selecting both peers and blocks. From these models, we obtain novel insights on the behavior of P2P swarming systems that motivate new mechanisms for publishers and peers to improve the overall performance. In particular, we obtain operational regions for swarm system. In addition, we show that system capacity significantly increases if publishers adopt the most deprived peer selection and peers reduce their service rates when they have all the file blocks but one.

==> TODO <==
2018

OK search for ???

OK double check 3.4

OK double check if throughput analysis sticks to K-tilde = 4, e.g., eq 20

OK align descriptions with those from infocom (and double check references)


Feb 2017




* results from Don about alternative policies

(possibly new appendix)

* polish last appendix, specially figs

(include exact system of non linear equations)

====


done:

* improve figure from tangram


* make sure we explain which curve was obtained with which model


* explain that the model cannot be used to infer lambdaS


* explain asymptotic U value in admission control, speciall when U=2 

* add admission control

* reference to dropbox

* reference to works by people from Argentina

*  explain mean field

* flow dynamics explanation



figure 2 needs to be cited in its section


adjust figures 1 and 2 for new definitions of lambdaC and lambdaS


add material to section 4.1 (including table)


make sure that we do not refer to infinite number of members in one-club (unboundedly etc) -- this is not the case => double check


remove infinte pop references => double check!
 

mention that in figure 2 we are showing the throughput of newcomers 


include observations about delay early on


finite population model already mentioned at section 4.1?  explain the rationale there

close section 4.1 with some remark about obtained result

adjust case pi=0 (can make probability arbitrarily close to 0 by increasing arrival rate)


====

2 July, 2015


* one goal of the paper: understanding throughput

* contributions


1) study of stability region of the system: stability region cahracterization. 
we discovered that there are two achievable thrughput regions: first,  the throuhghput
increases linearly with respect to the arrival rate.  When the arrival rate
achieves the threshold $lambda_s$, the throughput still increases but 
at the cost of infinite delays.  When the arrival rate grows beyond $lambda_c$
the throuhgput stabilizes.

2) system throuhgput upper bound

3) framework allows to evaluate the performance of policies that have been
previously proposed  in the
literature, including random peer selection and most deprived peer selection

4) our model and analysis suggests new policies.
 we analyze the proposed policies for increasing the throughput, 
 inclduing slowing down the rates for one club members and shielding newcomers.  
 we also show that admission control allows to further increase 
 the maximum achivable
  throughput.

* flow/story of paper

why studying the close system?

Finite population models have been used in the literature
to understand the behavior of queuing
networks as a function of the population size, and to study throughput under
saturation for large populations.    In what follows, we consider a finite
population model to validate the saturation throughput computed in Section 3.4. We
We show that for large population sizes, the throughput obtained with the finite
population model tends to $\lambda_s$. 
In the process, we discovered that in the finite population model a throughput
larger than  $\lambda_S$ might be achievable,
which indicates potential benefits of admission control.

TODO: in the whole paper, check for "saturation throughput" and "critical
throughput"


****************************


New results:

Open model simulation:

possible model 1 (truncation)
--- Poisson source, limited population size (capped at value suggested by Figure
7, roughly 125), arrival rate increasing from 6 to 8

*** expected results: 

cap with 100, 125, 150

as arrival rate increases, the departure
rate also increases.  saturates at some point. 


possible model 2 (queue waiting customers)
--- there is a queue of newcomers, and they join the system if
the population size is smaller than the admission control threshold N, otherwise
they wait 



****************************


--- analyze steady state probabilities of critical states (e.g., considering
Figure 7)

****************************

Future work (finite population size with inifinite one club?)

--- what happens when one club member completes download?

==========


September 9, 2016


I've just checked the p2p model generator,

 createmodel1.c 

at the following Dropbox folder,

~/Dropbox/p2p-stability/p2pmodelgenerator/p2pmodelgenerator-transient


*** added many comments ***


Currently, we are implementing admission control under the open (variable population size) model in simplest possible way:  whenever the population reaches a certain large size, arrivals do not occur.


1) check for the parameters

2) should we implement admission control in a different way?









==> discussion.tex <==
\section{Scalability of Peer-to-Peer Systems}
\label{sec:discussion}

In P2P systems every new peer entering a swarm brings additional resources
(transmission capacity and storage) since it acts both as a client and as a content 
provider. 
Therefore it is natural to expect  the overall system throughput to increase  
as the number of peers \daniel{increases.}  
However, the throughput growth is not unbounded.
Figure \ref{fig:limited-thr}, obtained from one of the models we developed,
illustrates this well.
%
\begin{figure}[htb]
\center
\includegraphics[scale=0.55]{plots/3mr00.250.50.5-1out01111011.eps}
\caption{Limited throughput as peer population grows.}
\label{fig:limited-thr}
\end{figure}
%
The figure shows that throughput grows almost linearly in the \eat{increase in } \daniel{size of} the swarm
population until it reaches a threshold ($\lambda_c$).
%and then slightly decreases and levels off.
Briefly, although the available resources increase with increasing number of peers,
they are not fully utilized.
For instance, this is the case where a peer has no block different from those that
its neighboring peers possess.

We have observed two operating regimes in the P2P systems
of interest to us.
The first is a \textit{stable} operating regime where all peers that arrive acquire
the content in a finite amount of time.  
Associated with this regime, we have a threshold $\lambda_s$ such that the system is stable
provided that the peer arrival rate $\lambda$ satisfies $\lambda < \lambda_s$.
\begin{comment}
For many resource constrained systems, $\lambda_s$ also corresponds to the
maximum possible throughput.
However, this does not appear to be the case in the P2P systems that we consider.  
In particular, 
if we let $\Upsilon(\lambda)$ denote the system throughput as a function of $\lambda$,
then it appears to be an increasing function of $\lambda$ satisfying 
$\Upsilon(\lambda) = \lambda$ for $\lambda < \lambda_s$ and 
$\lim_{\lambda \rightarrow \infty} \Upsilon(\lambda) = \lambda_s$.
\eat{ > \lambda_s. 
the throughput first increases as a function of $\lambda$ and then converges
to its limit $\lambda_s$.  } \eat{
then it appears to be a strictly increasing function of $\lambda$ satisfying 
$\Upsilon(\lambda) = \lambda$ for $\lambda < \lambda_s$ and
$\lim_{\lambda \rightarrow \infty} \Upsilon(\lambda) = \lambda_c > \lambda_s$.  }
\end{comment}
Then, our study points out that it is interesting to implement 
admission control, as in a closed system there is a second regime where the maximum achievable throughput, $\lambda_c$, 
can be larger than $\lambda_s$  (see Figure~\ref{fig:limited-thr}).  

\eat{
In particular, if we let $\Upsilon(\lambda)$ denote the system throughput as a 
function of $\lambda$,
then it appears to be a strictly increasing function of $\lambda$ satisfying 
$\Upsilon(\lambda) = \lambda$ for $\lambda < \lambda_s$ and
$\lim_{\lambda \rightarrow \infty} \Upsilon(\lambda) = \lambda_c > \lambda_s$.  
Note that $\lambda_c$ is a measure associated to the open system.  Our study points out that it is interesting to implement 
admission control, as in a closed system the throughput can be larger than $\lambda_s$.  
}

\eat{
\textcolor{red}{NOTE: this last limit has to be re-checked.
The limit $KU$ we show for open system depends on the server policy.
The overshoot in the curve occurs only in the closed system and we are able to achieve $\lambda_c$.
I believe this is expected, but the sentence we had before is not consistent and has to change.} 
\textcolor{red}{Also recheck the following sentence}.  }
%In what follows, we describe how to calculate these thresholds
%$\lambda_s$ and $\lambda_c$ for a variety of server and peer scheduling policies. 

We briefly explain the shape of the throughput curve of Figure \ref{fig:limited-thr}.
Assume a P2P system in which peers leave as soon as they complete downloads.
The file downloaded by a particular swarm is divided into $K$ equal size blocks.
Let $U$ be the server capacity \textit{that is allocated to the swarm} 
in blocks per time unit.  Let $\mu$ be the peers capacity.   
\eat{ (theneighbor and block selection policies adopted by the publisher and peers).   }
When the arrival rate of peers is large relative to $U$ the system will reach,
with high probability, a state in which all peers have all but one of the blocks
(say, block $X$). 
In this scenario, only the server has block $X$ and \eat{then} as soon as
a peer obtains the missing block $X$ from the server it leaves the system without
helping to serve block $X$ to others.
On the other hand, new peers that arrive are quickly served by their
peers and are able to obtain all blocks but $X$.
As a consequence, the system behaves approximately like a client server system:
peers depart \daniel{at}  rate $U$ since they do not cooperate to obtain the missing block.
In addition, although the available resources grow with the swarm size, these resources
are not fully~utilized.


The queueing model we propose in Section \ref{sec:models} to estimate the limiting throughput 
takes into account that, when the system is saturated, with high probability most peers in the system
eventually obtain all but the rarest block.
We also show that the limiting throughput depends on the service policies adopted by the server
and peers.

In a P2P system, the publisher needs to decide what block to transmit next \daniel{and} to
which peer.
Likewise, a peer has to decide what peer to contact and which block to request.
In the literature, it has been assumed that peers go through random encounters
and that peers are paired uniformly at
random~\cite{hajek, oguz2012stable, zhou2011stability}.
Nonetheless, if \eat{ peers strategically select their} \daniel{the publisher can strategically select its}  
neighbors, then  it is possible
to improve the overall system capacity.
Before introducing our models we first describe the policies that we consider.

Throughout this paper, we assume that peers select a neighbor uniformly at random
at every transmission opportunity to exchange blocks (random peer selection).
We also consider the case where trackers dynamically \eat{ provide } \daniel{inform} 
each peer $P$ of the set of peers in the swarm in need of blocks owned by $P$. 
In this case, peers can select their neighbors uniformly at random among those 
that need the blocks they possess.
We refer to this neighbor selection policy as random \emph{useful} peer selection.

After choosing a neighbor, each peer selects
one of its blocks for transmission to the neighbor.
If the block is selected uniformly at random, the policy is referred to as random useful
block selection.
If peers have access to a list of the number of replicas of each block, they can build a
rarest-block set containing the indices of the blocks with the least number of copies in
the swarm~\cite{legout:07}.
This set can then be used by peers to select which block to transmit.
This policy is referred to as rarest first block selection. 

The publisher can select its peers and blocks in the same way as the peers.
In addition, the publisher can also select its peers using the most deprived policy.
Under this policy, the publisher prioritizes sending blocks to peers that own the least
amount of blocks among those in the swarm.  
If the arrival rate of peers is large (or the swarm size is large) these peers are likely
to be content-less peers, also referred to as newcomers. 
%The rationale behind the most deprived policy is to transmit rare blocks to peers
%that will linger longer in the system and as such will
%have more time to distribute the rarest blocks throughout the swarm.
Table \ref{tab:policies} summarizes these policies.

\begin{table}
\scriptsize
\center
\begin{tabular}{l|l}
\hline
peers & publisher \\
\hline \hline
random peer/random useful block (RP/RUB) & random peer/random useful block  (RP/RUB) \\
random peer/rarest first block (RP/RFB) & random peer/rarest first block (RP/RFB) \\
random useful peer/random useful block (RUP/RUB) & most deprived peer/rarest first block (MDP/RFB)        \\
random peer/random useful block (RP/RUB) & most deprived peer/rarest first block (MDP/RFB)        \\
\hline
\end{tabular}
\caption{Neighbor and block selection policies} \label{tab:policies}
\end{table}


==> don_comments <==
I would like to suggest a revision.  I think that the reader will understand the model better if we don't introduce approximations until after we describe it.  This includes including F_i up to the maximum (K, K-1, K-2?) and similarly G_i.  I think this will make it easier for the reader to understand what is going on.  We can then state that little accuracy is lost by truncating the sequences F_i and G_i with the benefit of increased computational efficiency; BTW, is this true?

The other approximation is of s\mu' + UI(n_0=0, ...) by s\mu' + UP(N_0=0, n_1=0, ...).  I am comfortable with how it is introduced but I would wait until the exact model is described before introducing it.


Regarding the scalability paper.

1.  Are we the first to identify these three operating regimes, stable, linear throughput, unstable, growing throughput, unstable, constant throughput?  If so, we may want to highlight in intro.

2.  Section 2 focuses on P2P systems and their behavior but Figure 2 focuses on models.  DO we need Figure two and its description?  Doesn't Figure 1 summarize the three regimes?



